Understanding Bird's-Eye View of Road Semantics using an Onboard Camera

Autonomous navigation requires scene understanding of the action-space to move or anticipate events. For planner agents moving on the ground plane, such as autonomous vehicles, this translates to scene understanding in the bird's-eye view (BEV). However, the onboard cameras of autonomous cars are customarily mounted horizontally for a better view of the surrounding. In this work, we study scene understanding in the form of online estimation of semantic BEV maps using the video input from a single onboard camera. We study three key aspects of this task, image-level understanding, BEV level understanding, and the aggregation of temporal information. Based on these three pillars we propose a novel architecture that combines these three aspects. In our extensive experiments, we demonstrate that the considered aspects are complementary to each other for BEV understanding. Furthermore, the proposed architecture significantly surpasses the current state-of-the-art. Code: https://github.com/ybarancan/BEV_feat_stitch.

==> Iccv_plans.tex <==
1. Objects <Resolved with 17.6 mIOU>
-- Boundary loss does not help! -> smoothing + L1?
-- Adv.
-- Attention 
2. Argoverse results 
-- In progress 
3. Resnet
-- Supp.
4. Causality
-- Supp.
 <smaller frame gap!>
 
 =======================
 Minor changes;
1. Improve fig 2
2. Writing: HD-map semantics or BEV semantics
3. 
 

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> experiments.tex <==

\section{Experiments}
% \subsection{Implementation Details}

% We implemented our network in Tensorflow and used ADAM optimizer \cite{DBLP:journals/corr/KingmaB14} with a learning rate of $10^{-5}$. During the training, we use $N = 4$ frames (one past and two future frames) and time interval between consecutive frames is randomly sampled between one and three frames. This lets the network better handle different speeds in motion and acts as a data augmentation. %The method runs with 21FPS on a RTX 2080 Ti with an image size of ($448\times 800$).
% % \cite{tensorflow2015-whitepaper}

We implemented our network in Tensorflow. During the training, we use $N = 4$ frames (one past and two future frames) and time interval between consecutive frames is randomly sampled between one and three frames. This lets the network better handle different speeds in motion and acts as a data augmentation. %The method runs with 21FPS on a RTX 2080 Ti with an image size of ($448\times 800$).
% \cite{tensorflow2015-whitepaper}

\subsection{Datasets}

In our experiments, we use the NuScenes \cite{nuscenes2019} and Argoverse \cite{DBLP:conf/cvpr/ChangLSSBHW0LRH19} datasets. NuScenes consists of 1000 sequences recorded in Boston and Singapore. The sequences are annotated at 2Hz and the dataset provides rich semantic HD-maps with static BEV segmentations such as drivable area, pedestrian crossing, and walkways. The dataset also provides 3D bounding boxes of 23 object classes. For our experiments, we select six HD-map classes and for dynamic objects, we follow \cite{DBLP:conf/cvpr/RoddickC20} and select 10 object classes. We only use the front camera for training and evaluation. 

We also conducted experiments on the Argoverse dataset which has 65 training and 24 validation sequences. In Argoverse the sequences are annotated at 10Hz. Unlike NuScenes, Argoverse only provides drivable area as a static HD-map class. For dynamic objects we again follow \cite{DBLP:conf/cvpr/RoddickC20}.



% Unlike NuScenes, Argoverse does not provide rich semantic HD-maps\footnote{Argoverse provides HD-maps but these are focused on lane graphs.}, drivable area being the only static HD-map class. For dynamic objects we again follow \cite{DBLP:conf/cvpr/RoddickC20}.

\begin{table}[h]
% \caption{NuScenes Static Class only results}
\vspace{-1em}
\tabcolsep=0.11cm
\scriptsize{
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| }
% \hline
\rotatebox{50}{Model} & \rotatebox{50}{drivable} & \rotatebox{50}{ped cross} & \rotatebox{50}{walkway} & \rotatebox{50}{carpark}  & \rotatebox{50}{road} & \rotatebox{50}{lane} & \rotatebox{50}{occ} & \rotatebox{50}{4-Mean} & \rotatebox{50}{7-Mean} \\
\hline
% LSS$^*$ & 72.9 & -  & - & - & - & -& -& - & -\\ 
PON & 60.4 & 28.0  & 31.0 & 18.4 & - & -& -& 34.5 & -\\ 
Deeplab & 58.9 & 14.3  & 19.1 & 21.2 & 55.0 & 40.4 & 48.0 & 28.4 & 36.7 \\
Ours & \textbf{72.9} & \textbf{31.2}  & \textbf{36.9} & \textbf{27.1} & \textbf{73.0} & \textbf{51.7} &
\textbf{61.1} & \textbf{42.0} & \textbf{50.6} \\ 
Ours(F) & 68.6 & 27.0  & 30.5 & 24.5 & 71.5 & 49.9 &
\textbf{61.1} & 37.6 & 47.6 \\ 
\hline
\end{tabular}
\end{center}
}
\vspace{-1em}
\caption{NuScenes static class only experiments are done in two settings. In the standard setting, results are evaluated only for non-occluded pixels. In the (F) FOV setting, every pixel in field-of-view is considered. Since our method processes videos, it can deal with occlusion. Our method surpasses the baselines in both settings, producing better results even when occluded pixels are considered.}
\vspace{-1em}
\label{tab:nuscenes_bev_results}
\end{table}


% \begin{table*}[h]
% % \caption{NuScenes Static Class only results}
% \vspace{-2em}
% \tabcolsep=0.11cm
% \scriptsize{
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| }
% \hline
% Model & drivable & ped cross & walkway & carpark  & road segment & lane & occlusion & 4-Mean & 7-Mean \\
% \hline
% % LSS$^*$ & 72.9 & -  & - & - & - & -& -& - & -\\ 
% PON & 60.4 & 28.0  & 31.0 & 18.4 & - & -& -& 34.5 & -\\ 
% Deeplab-v3+ & 58.9 & 14.3  & 19.1 & 21.2 & 55.0 & 40.4 & 48.0 & 28.4 & 36.7 \\
% Ours & \textbf{72.9} & \textbf{31.2}  & \textbf{36.9} & \textbf{27.1} & \textbf{73.0} & \textbf{51.7} &
% \textbf{61.1} & \textbf{42.0} & \textbf{50.6} \\ 
% Ours - FOV & 68.6 & 27.0  & 30.5 & 24.5 & 71.5 & 49.9 &
% \textbf{61.1} & 37.6 & 47.6 \\ 
% \hline
% \end{tabular}
% \end{center}
% }
% \caption{NuScenes static class only experiments are evaluated in two settings. In the standard setting the results are evaluated only for non-occluded pixels. In the FOV setting, every pixel in field-of-view is considered. Since our method processes videos, it can deal with occlusion. Our method surpasses the baselines in both settings, producing better results even when occluded pixels are considered.}
% \vspace{-1em}
% \label{tab:nuscenes_bev_results}
% \end{table*}

\subsection{Data Generation} \label{subsection:data_generation}
To provide a fair comparison with baselines, we followed the setup of Pyramid Occupancy Network \cite{DBLP:conf/cvpr/RoddickC20}. We used the same train/val split which is specially selected to provide a more challenging and representative sample distribution for the evaluation. We also used the same BEV lattice grid with a 0.25m resolution that spans a region of $[-25,25]$m in lateral and $[1,50]$m in longitudinal direction. Note that all our BEV labels are represented in this BEV grid. We also use the same occlusion masks to report the results.

% In order to obtain more accurate results, we use the LIDAR scans to estimate the height of the surfaces.
Generating the lBEV labels for the static classes is straightforward since the datasets directly provide this data. To obtain the static image-level labels, we warp BEV labels onto the image plane. For the objects, we consider the ground plane projection of the 3D bounding boxes as the BEV labels of the object. Since we specifically want the image branch to estimate ground projections, we can obtain image-level labels by projecting these BEV labels to the image plane. 


\subsection{Baselines}
\label{subsec:exp_abl}
To evaluate the performance of our method, we selected several baselines. The first baseline is a modified Deeplabv3+ \cite{deeplabv3plus2018} network that is pre-trained on Cityscapes \cite{Cordts2016Cityscapes}. We modified the final layers to match the number of classes and added a small sub-network for occlusion segmentation. The modified network is trained on NuScenes. The network outputs the image level segmentation, which we warp to the BEV plane using the ground truth projections. The second baseline is the SOTA method, Pyramid Occupancy Network (PON) \cite{DBLP:conf/cvpr/RoddickC20}. Finally, we also compare to Variational Encoder-Decoder Network (VED) \cite{DBLP:journals/ral/LuMD19} and View Parser Network (VPN) \cite{DBLP:journals/ral/PanSLAZ20} which generally perform worse than PON. As an additional baseline, we use our single frame network to obtain framewise BEV estimations. We then aggregate these estimations by warping them to the BEV reference frame and combining them by averaging, considering the individual visibility masks. This lets us benchmark our temporal aggregation module against the post-processing. We refer to this baseline as \emph{Post} in Tab.~\ref{tab:nuscenes_object_abla}.



